Sparse Matrix-Based HPC Tomography

Tomographic imaging has benefited from advances in X-ray sources, detectors and optics to enable novel observations in science, engineering and medicine. These advances have come with a dramatic increase of input data in the form of faster frame rates, larger fields of view or higher resolution, so high performance solutions are currently widely used for analysis. Tomographic instruments can vary significantly from one to another, including the hardware employed for reconstruction: from single CPU workstations to large scale hybrid CPU/GPU supercomputers. Flexibility on the software interfaces and reconstruction engines are also highly valued to allow for easy development and prototyping. This paper presents a novel software framework for tomographic analysis that tackles all aforementioned requirements. The proposed solution capitalizes on the increased performance of sparse matrix-vector multiplication and exploits multi-CPU and GPU reconstruction over MPI. The solution is implemented in Python and relies on CuPy for fast GPU operators and CUDA kernel integration, and on SciPy for CPU sparse matrix computation. As opposed to previous tomography solutions that are tailor-made for specific use cases or hardware, the proposed software is designed to provide flexible, portable and high-performance operators that can be used for continuous integration at different production environments, but also for prototyping new experimental settings or for algorithmic development. The experimental results demonstrate how our implementation can even outperform state-of-the-art software packages used at advanced X-ray sources worldwide.

==> Sections/implementation.tex <==

$$\cdots$$
%Fast Radon and inverse Radon transforms form the computational kernels of many image reconstruction algorithms. The 2D Radon tranform of an image x can be implemented in a number of ways. One of the most efficient ways to perform Radon{x} is to first perform a 2D FFT of x on a regular grid, and then interpolate the transform onto a polar grid before 1D inverse Fourier transforms are applied to interpolated points along the same radial lines. The interpolation between the Cartesian and polar grid is the key step in this procedure. It can be carried out using a “gridding” algorithm that maintains the desired accuracy with low computational complexity. The gridding algorithm essentially allows us to perform a non-uniform FFT. The gridding operation requires the convolution between irregular samples and a kernel calculated at regular sample position and vice versa (Fig. 5 and [3]). [plagiarized from myself -sm]
